Reconstruction of space-dependence and nonlinearity of a reaction term in a subdiffusion equation

In this paper we study the simultaneous reconstruction of two coefficients in a reaction-subdiffusion equation, namely a nonlinearity and a space dependent factor. The fact that these are coupled in a multiplicative matter makes the reconstruction particularly challenging. Several situations of overposed data are considered: boundary observations over a time interval, interior observations at final time, as well as a combination thereof. We devise fixed point schemes and also describe application of a frozen Newton method. In the final time data case we prove convergence of the fixed point scheme as well as uniqueness of both coefficients. Numerical experiments illustrate performance of the reconstruction methods, in particular dependence on the differentiation order in the subdiffusion equation.

==> figure_driver.tex <==

\noindent
% Pictures for the Inverse problem of Recovering a Spatial Coefficient and the
% Nonlinear Reaction Term in a Parabolic Equation.

\newdimen\xfigdim \newdimen\yfigdim \newdimen\legendheight
\newdimen\xfiglenshort \newdimen\yfiglenshort
\xfigdim = 1.85true in
\yfigdim = 45true in
\legendheight = 0.16true in
%
\setbox\figurelegend=\hbox{
\beginpicture
  \setcoordinatesystem units <0.33\xfigdim,0.7\legendheight> %point at 0 -0.7
  \setplotarea x from 0 to 2, y from 0 to 3
\footnotesize
\linethickness=0.5pt
\scriptsize
   %\setdashes <3pt>  \putrule from 0 3 to 1.25 3
   \setsolid
   \Black{\relax \putrule from 0 6 to 0.5 6 \relax}\relax
   \put {actual}  [l] at 0.6 6
%
   \setdashes <2pt>
   \Red{\relax \putrule from 0 5 to 0.5 5 \relax}\relax
   \put {iter 2\, / \hspace*{0.9mm} 3 } [l] at 0.6 5
%
   \setdashes <5pt>
   \Green{\relax \putrule from 0 4 to 0.5 4 \relax}\relax
   \put {iter 3\, / \,10 } [l] at 0.6 4
%
   \setdashes <8pt>
   \Blue{\relax \putrule from 0 3 to 0.5 3 \relax}\relax
   \put {iter 9\, / \,30 } [l] at 0.6 3
%
\endpicture
}
\setbox\figurelegendvalues=\vbox{
\beginpicture
  \setcoordinatesystem units <0.33\xfigdim,\legendheight> %point at 0 -0.7
  \setplotarea x from 0 to 2, y from 0 to 1.5
\footnotesize
\put {$q_{init}(x) = 0$} at 0 0.0

\put {$f_{init}(u) = 4u$} at 0  1.0
\endpicture
}
%
\setbox\figurelegendtext=\vbox{
\beginpicture
  \setcoordinatesystem units <0.33\xfigdim,\legendheight> %point at 0 -0.7
  \setplotarea x from 0 to 8, y from 0 to 3
\footnotesize
\put{Row 1: $q$ from final time data} [l] at 0 3
\put{Row 2: $q$ from mixed data} [l] at 0 2
\put{Row 3: $f$ from final time data} [l] at 0 1
\put{Row 4: $f$ from mixed data} [l] at 0 0
\put{Column 1: $\alpha = 0.5$} [l] at 4 3
\put{Column 2: $\alpha = 0.7$} [l] at 4 2
\put{Column 3: $\alpha = 0.99$} [l] at 4 1
\endpicture
}
%
%\hbox to\hsize{\copy\figurelegendtext}
\hbox to\hsize{\copy\figurelegendtext\hss\raise0.22true in\copy\figurelegendvalues\hss\lower 1em\copy\figurelegend\hss}
%
\setbox\figureone=\vbox{\hsize=\xfiglen   % This box is for q_fiti_alpha=0.5
% colours follow those of the matlab pictures
% This is for fixed point scheme and $q(x)$, $\alpha = 0.5$
\beginpicture
\scriptsize
  \setcoordinatesystem units <\xfigdim,\yfigdim>  point at 0 -1.5
  \setplotarea x from 0 to 1, y from 0 to 0.025
  \axis bottom shiftedto y=0 ticks short numbered from 0 to 1 by 0.2 /
  %\axis left ticks short unnumbered from 0 to 0.02 by 0.01 /
  \axis left ticks short unlabeled from 0 to 0.025 by 0.005 /
  \put {0.25} [l] at 0.02 0.025
  %\put{{\sevenrm All $\times 10^{-3}$}} left at 0.02 1.5
  %\put {{\sevenrm $q_{err}$, $\alpha=0.99$}} [rb] at 0.96 0.05
\setquadratic
\setsolid
\Black{\relax  % exact values
%\setdots
\plot
        0          0
    0.0500    0.0048
    0.1000    0.0090
    0.1500    0.0127
    0.2000    0.0160
    0.2500    0.0188
    0.3000    0.0210
    0.3500    0.0227
    0.4000    0.0240
    0.4500    0.0248
    0.5000    0.0250
    0.5500    0.0248
    0.6000    0.0240
    0.6500    0.0227
    0.7000    0.0210
    0.7500    0.0188
    0.8000    0.0160
    0.8500    0.0128
    0.9000    0.0090
    0.9500    0.0048
    1.0000         0
/
}
%
\Blue{\relax
\setdashes <8pt>
\plot
    0.0000    0.0001 
    0.0500    0.0047
    0.1000    0.0089
    0.1500    0.0126
    0.2000    0.0158
    0.2500    0.0186
    0.3000    0.0208
    0.3500    0.0225
    0.4000    0.0237
    0.4500    0.0245
    0.5000    0.0247
    0.5500    0.0245
    0.6000    0.0237
    0.6500    0.0225
    0.7000    0.0208
    0.7500    0.0185
    0.8000    0.0158
    0.8500    0.0126
    0.9000    0.0089
    0.9500    0.0047
    1.0000         0
/
 }\relax
%
% This looks like magenta in matlab plots
\Green{\relax 
\setdashes <5pt>
\plot
    0.0000   -0.0002  
    0.0500    0.0046 
    0.1000    0.0088
    0.1500    0.0125
    0.2000    0.0158
    0.2500    0.0185
    0.3000    0.0207
    0.3500    0.0225
    0.4000    0.0237
    0.4500    0.0245
    0.5000    0.0247
    0.5500    0.0245
    0.6000    0.0238
    0.6500    0.0225
    0.7000    0.0208
    0.7500    0.0186
    0.8000    0.0159
    0.8500    0.0126
    0.9000    0.0089
    0.9500    0.0047
    1.0000         0
/
 }\relax
%
\Red{\relax 
\setdashes <2pt>
\plot
    0.0000  -0.0009       
    0.0500   0.0041    
    0.1000   0.0085   
    0.1500   0.0124  
    0.2000   0.0158 
    0.2500   0.0187 
    0.3000   0.0211
    0.3500   0.0229
    0.4000   0.0242
    0.4500   0.0251  
    0.5000   0.0254 
    0.5500   0.0251
    0.6000   0.0244 
    0.6500   0.0232
    0.7000   0.0214 
    0.7500   0.0191
    0.8000   0.0163  
    0.8500   0.0130 
    0.9000   0.0092
    0.9500   0.0049
    1.0000        0
/
}\relax
%
\endpicture
}   
%
\setbox\figuretwo=\vbox{\hsize=\xfiglen   % This box is for q_fiti_alpha=0.7
% colours follow those of the matlab pictures
% This is for fixed point scheme and $q(x)$, $\alpha = 0.7$
\beginpicture
\scriptsize
  \setcoordinatesystem units <\xfigdim,\yfigdim>  point at 0 -1.5
  \setplotarea x from 0 to 1, y from 0 to 0.025
  \axis bottom shiftedto y=0 ticks short numbered from 0 to 1 by 0.2 /
  %\axis left ticks short numbered from 0 to 0.02 by 0.01 /
  %\axis left ticks unlabeled from 0 to 0.025 by 0.005 /
  \axis left ticks short unlabeled from 0 to 0.025 by 0.005 /
  \put {0.25} [l] at 0.02 0.025
  %\put{{\sevenrm All $\times 10^{-3}$}} left at 0.02 1.5
  %\put {{\sevenrm $q_{err}$, $\alpha=0.99$}} [rb] at 0.96 0.05
\setquadratic
\Black{\relax  % exact values
\setsolid
\plot
        0          0
    0.0500    0.0048
    0.1000    0.0090
    0.1500    0.0127
    0.2000    0.0160
    0.2500    0.0188
    0.3000    0.0210
    0.3500    0.0227
    0.4000    0.0240
    0.4500    0.0248
    0.5000    0.0250
    0.5500    0.0248
    0.6000    0.0240
    0.6500    0.0227
    0.7000    0.0210
    0.7500    0.0188
    0.8000    0.0160
    0.8500    0.0128
    0.9000    0.0090
    0.9500    0.0048
    1.0000         0
/\relax
}\relax
%
\Blue{\relax
\setdashes <8pt>
\plot
0.0000  0.0001
0.0500  0.0048
0.1000  0.0090
0.1500  0.0127
0.2000  0.0159
0.2500  0.0186
0.3000  0.0208
0.3500  0.0225
0.4000  0.0238
0.4500  0.0245
0.5000  0.0247
0.5500  0.0245
0.6000  0.0237
0.6500  0.0225
0.7000  0.0208
0.7500  0.0185
0.8000  0.0158
0.8500  0.0126
0.9000  0.0089
0.9500  0.0047
1.0000  0
/\relax
}\relax
%
% This looks like magenta in matlab plots
\Green{\relax 
\setdashes <5pt>
\plot
0.0000  -0.0002
0.0500  0.0046
0.1000  0.0088
0.1500  0.0126
0.2000  0.0158
0.2500  0.0186
0.3000  0.0208
0.3500  0.0226
0.4000  0.0238
0.4500  0.0246
0.5000  0.0248
0.5500  0.0246
0.6000  0.0239
0.6500  0.0226
0.7000  0.0209
0.7500  0.0186
0.8000  0.0159
0.8500  0.0127
0.9000  0.0090
0.9500  0.0047
1.0000   0
/\relax
}\relax
%
\setsolid
\Red{\relax 
\setdashes <2pt>
\plot
0.0000  -0.0011
0.0500  0.0040
0.1000  0.0085
0.1500  0.0125
0.2000  0.0160
0.2500  0.0189
0.3000  0.0214
0.3500  0.0233
0.4000  0.0246
0.4500  0.0255
0.5000  0.0258
0.5500  0.0256
0.6000  0.0248
0.6500  0.0236
0.7000  0.0218
0.7500  0.0195
0.8000  0.0166
0.8500  0.0133
0.9000  0.0094
0.9500  0.0049
1.0000   0
/\relax}\relax
\endpicture
}
%
\setbox\figurethree=\vbox{\hsize=\xfiglen   % This box is for q_fiti_alpha=0.99
% colours follow those of the matlab pictures
% This is for fixed point scheme and $q(x)$, $\alpha = 0.99$
\beginpicture
\scriptsize
  \setcoordinatesystem units <\xfigdim,\yfigdim>  point at 0 -1.5
  \setplotarea x from 0 to 1, y from 0 to 0.025
  \axis bottom shiftedto y=0 ticks short numbered from 0 to 1 by 0.2 /
  \axis left ticks short unlabeled from 0 to 0.025 by 0.005 /
  \put {0.25} [l] at 0.02 0.025
  %\axis left ticks unlabeled from 0 to 0.025 by 0.005 /
  %\put{{\sevenrm All $\times 10^{-3}$}} left at 0.02 1.5
  %\put {{\sevenrm $q_{err}$, $\alpha=0.99$}} [rb] at 0.96 0.05
\setquadratic
\setdashes <3pt>
\setsolid
\Black{\relax  % exact values
\plot
0         0
0.0500    0.0048
0.1000    0.0090
0.1500    0.0127
0.2000    0.0160
0.2500    0.0188
0.3000    0.0210
0.3500    0.0227
0.4000    0.0240
0.4500    0.0248
0.5000    0.0250
0.5500    0.0248
0.6000    0.0240
0.6500    0.0227
0.7000    0.0210
0.7500    0.0188
0.8000    0.0160
0.8500    0.0128
0.9000    0.0090
0.9500    0.0048
1.0000         0
/\relax
}
%
\Blue{\relax
\setdashes <8pt>
\plot
0.0000 -0.0002
0.0500 0.0046
0.1000 0.0088
0.1500 0.0126
0.2000 0.0159
0.2500 0.0186
0.3000 0.0209
0.3500 0.0226
0.4000 0.0239
0.4500 0.0247
0.5000 0.0249
0.5500 0.0247
0.6000 0.0239
0.6500 0.0227
0.7000 0.0210
0.7500 0.0187
0.8000 0.0160
0.8500 0.0127
0.9000 0.0090
0.9500 0.0047
1.0000  0
/\relax
}
\Green{\relax 
\setdashes <5pt>
\plot
0.0000 0.0002
0.0500 0.0049
0.1000 0.0091
0.1500 0.0128
0.2000 0.0160
0.2500 0.0188
0.3000 0.0210
0.3500 0.0227
0.4000 0.0239
0.4500 0.0247
0.5000 0.0249
0.5500 0.0246
0.6000 0.0239
0.6500 0.0226
0.7000 0.0209
0.7500 0.0186
0.8000 0.0159
0.8500 0.0127
0.9000 0.0089
0.9500 0.0047
1.0000 0
 /\relax
}
%\relax
%\setplotsymbol({\fiverm $\bullet$})
\Red{\relax 
\setdots
\setdashes <2pt>
\plot
0.0000 -0.0018
0.0500 0.0034
0.1000 0.0081
0.1500 0.0122
0.2000 0.0158
0.2500 0.0188
0.3000 0.0213
0.3500 0.0233
0.4000 0.0247
0.4500 0.0256
0.5000 0.0259
0.5500 0.0258
0.6000 0.0250
0.6500 0.0238
0.7000 0.0220
0.7500 0.0197
0.8000 0.0168
0.8500 0.0134
0.9000 0.0095
0.9500 0.0050
1.0000 0
/\relax
}
\endpicture
%
}
\hbox to \hsize{\copy\figureone\hss\copy\figuretwo\hss\copy\figurethree}
\vskip 15pt
%\bigskip
%\end{document}
%%%%%%%%%%%%%%%%%%%%%%%  end of q_fiti plots  %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%  beginning of q_mixed plots  %%%%%%%%%%%%%%%%%%%%
\yfigdim = 2.25true in
\setbox\figurefour=\vbox{\hsize=\xfiglen   % This box is for q_mixed alpha=0.5
% colours follow those of the matlab pictures
% This is for mixed scheme and $q(x)$, $\alpha = 0.5$
\beginpicture
\scriptsize
  \setcoordinatesystem units <\xfigdim,\yfigdim>  point at 0 -0.4
  \setplotarea x from 0 to 1, y from -0.4 to 0.2
  \axis bottom shiftedto y=0 ticks short numbered from 0 to 1 by 0.2 /
  \axis left ticks short unlabeled from -0.4 to 0.2 by 0.2 /
  \put {0.2} [l] at 0.02 0.2
  \put {-0.2} [l] at 0.02 -0.2
  \put {-0.4} [l] at 0.02 -0.4
  %\axis left ticks short numbered from 0 to 0.02 by 0.01 /
%\put{{\sevenrm All $\times 10^{-3}$}} left at 0.02 1.5
  %\put {{\sevenrm $q_{err}$, $\alpha=0.5$}} [rb] at 0.96 0.05
\setquadratic
\setdashes <3pt>
\setsolid
\Black{\relax  % exact values
%\setdots
\plot
0.0000  0.0
0.0500  0.0238
0.1000  0.0450
0.1500  0.0638
0.2000  0.0800
0.2500  0.0938
0.3000  0.1050
0.3500  0.1137
0.4000  0.1200
0.4500  0.1238
0.5000  0.1250
0.5500  0.1237
0.6000  0.1200
0.6500  0.1137
0.7000  0.1050
0.7500  0.0938
0.8000  0.0800
0.8500  0.0638
0.9000  0.0450
0.9500  0.0238
1.0000  0
/\relax
}\relax
%
\Blue{\relax
\setdashes <8pt>
\plot
0.0000  0.0002
0.0500  0.0238
0.1000  0.0450
0.1500  0.0636
0.2000  0.0798
0.2500  0.0935
0.3000  0.1047
0.3500  0.1134
0.4000  0.1196
0.4500  0.1233
0.5000  0.1245
0.5500  0.1233
0.6000  0.1196
0.6500  0.1133
0.7000  0.1046
0.7500  0.0934
0.8000  0.0797
0.8500  0.0635
0.9000  0.0448
0.9500  0.0237
1.0000  0
/\relax
}\relax
%
% This looks like magenta in matlab plots
\Green{\relax 
\setdashes <5pt>
\plot
0.0000  0.0450
0.0500  0.0518
0.1000  0.0577
0.1500  0.0627
0.2000  0.0667
0.2500  0.0697
0.3000  0.0717
0.3500  0.0728
0.4000  0.0730
0.4500  0.0722
0.5000  0.0704
0.5500  0.0677
0.6000  0.0640
0.6500  0.0593
0.7000  0.0537
0.7500  0.0472
0.8000  0.0397
0.8500  0.0312
0.9000  0.0217
0.9500  0.0114
1.0000  0
/\relax
}\relax
%
\Red{\relax 
\setdashes <2pt>
\plot
0.0000  -0.3714
0.0500  -0.3711
0.1000  -0.3688
0.1500  -0.3646
0.2000  -0.3585
0.2500  -0.3505
0.3000  -0.3406
0.3500  -0.3287
0.4000  -0.3150
0.4500  -0.2993
0.5000  -0.2817
0.5500  -0.2621
0.6000  -0.2407
0.6500  -0.2173
0.7000  -0.1920
0.7500  -0.1648
0.8000  -0.1357
0.8500  -0.1046
0.9000  -0.0717
0.9500  -0.0368
1.0000  0
/\relax
}\relax
%
\endpicture
}   
%
%\vfill\eject
%\copy\figurefour
%\end{document}
%
\setbox\figurefive=\vbox{\hsize=\xfiglen   % This box is for q_fiti_alpha=0.7
% colours follow those of the matlab pictures
% This is for fixed point scheme and $q(x)$, $\alpha = 0.7$
\beginpicture
\scriptsize
  \setcoordinatesystem units <\xfigdim,\yfigdim>  point at 0 -1.5
  \setplotarea x from 0 to 1, y from -0.4 to 0.2
  \axis bottom shiftedto y=0 ticks short numbered from 0 to 1 by 0.2 /
  \axis left ticks short unlabeled from -0.4 to 0.2 by 0.2 /
  \put {0.2} [l] at 0.02 0.2
  \put {-0.2} [l] at 0.02 -0.2
  \put {-0.4} [l] at 0.02 -0.4
  %\axis left ticks short numbered from -0.4 to 0.2 by 0.2 /
  %\put{{\sevenrm All $\times 10^{-3}$}} left at 0.02 1.5
  %\put {{\sevenrm $q_{err}$, $\alpha=0.99$}} [rb] at 0.96 0.05
\setquadratic
\setdashes <3pt>
\setsolid
\Black{\relax  % exact values
\plot
0.0000  0.0000
0.0500  0.0238
0.1000  0.0450
0.1500  0.0638
0.2000  0.0800
0.2500  0.0938
0.3000  0.1050
0.3500  0.1137
0.4000  0.1200
0.4500  0.1238
0.5000  0.1250
0.5500  0.1237
0.6000  0.1200
0.6500  0.1137
0.7000  0.1050
0.7500  0.0938
0.8000  0.0800
0.8500  0.0638
0.9000  0.0450
0.9500  0.0238
1.0000  0.0000
/\relax
}\relax
%
\Blue{\relax
\setdashes <8pt>
\plot
0.0000  0.0003
0.0500  0.0239
0.1000  0.0450
0.1500  0.0637
0.2000  0.0799
0.2500  0.0935
0.3000  0.1047
0.3500  0.1134
0.4000  0.1196
0.4500  0.1234
0.5000  0.1246
0.5500  0.1233
0.6000  0.1196
0.6500  0.1133
0.7000  0.1046
0.7500  0.0934
0.8000  0.0797
0.8500  0.0635
0.9000  0.0448
0.9500  0.0237
1.0000  0
/\relax
}\relax
%
% This looks like magenta in matlab plots
\Green{\relax 
\setdashes <5pt>
\plot
0.0000  0.0442
0.0500  0.0488
0.1000  0.0526
0.1500  0.0558
0.2000  0.0582
0.2500  0.0599
0.3000  0.0610
0.3500  0.0613
0.4000  0.0608
0.4500  0.0597
0.5000  0.0578
0.5500  0.0553
0.6000  0.0520
0.6500  0.0480
0.7000  0.0433
0.7500  0.0379
0.8000  0.0317
0.8500  0.0249
0.9000  0.0173
0.9500  0.0090
1.0000  0.0000
/\relax
}\relax
%
\Red{\relax 
\setdashes <2pt>
\plot
0.0000  -0.3287
0.0500  -0.3491
0.1000  -0.3657
0.1500  -0.3783
0.2000  -0.3871
0.2500  -0.3921
0.3000  -0.3931
0.3500  -0.3902
0.4000  -0.3835
0.4500  -0.3729
0.5000  -0.3584
0.5500  -0.3400
0.6000  -0.3178
0.6500  -0.2916
0.7000  -0.2616
0.7500  -0.2277
0.8000  -0.1899
0.8500  -0.1483
0.9000  -0.1027
0.9500  -0.0533
1.0000   0.0000
/\relax
}\relax
\endpicture
}
%
\setbox\figuresix=\vbox{\hsize=\xfiglen   % This box is for q_fiti_alpha=0.99
% colours follow those of the matlab pictures
% This is for fixed point scheme and $q(x)$, $\alpha = 0.99$
\beginpicture
\scriptsize
  \setcoordinatesystem units <\xfigdim,\yfigdim>  point at 0 -1.5
  \setplotarea x from 0 to 1, y from -0.4 to 0.2
  \axis bottom shiftedto y=0 ticks short numbered from 0 to 1 by 0.2 /
  \axis left ticks short unlabeled from -0.4 to 0.2 by 0.2 /
  \put {0.2} [l] at 0.02 0.2
  \put {-0.2} [l] at 0.02 -0.2
  \put {-0.4} [l] at 0.02 -0.4
  %\axis left ticks short numbered from -0.4 to 0.2 by 0.2 /
  %\put{{\sevenrm All $\times 10^{-3}$}} left at 0.02 1.5
  %\put {{\sevenrm $q_{err}$, $\alpha=0.99$}} [rb] at 0.96 0.05
\setquadratic
\setdashes <3pt>
\setsolid
\Black{\relax  % exact values
\plot
0.0000  0.0
0.0500  0.0238
0.1000  0.0450
0.1500  0.0638
0.2000  0.0800
0.2500  0.0938
0.3000  0.1050
0.3500  0.1137
0.4000  0.1200
0.4500  0.1238
0.5000  0.1250
0.5500  0.1237
0.6000  0.1200
0.6500  0.1137
0.7000  0.1050
0.7500  0.0938
0.8000  0.0800
0.8500  0.0638
0.9000  0.0450
0.9500  0.0238
1.0000  0
/\relax
}\relax
%
\Blue{\relax
\setdashes <8pt>
\plot
0.0000  0.0001
0.0500  0.0238
0.1000  0.0450
0.1500  0.0637
0.2000  0.0799
0.2500  0.0936
0.3000  0.1048
0.3500  0.1136
0.4000  0.1198
0.4500  0.1236
0.5000  0.1248
0.5500  0.1235
0.6000  0.1198
0.6500  0.1136
0.7000  0.1048
0.7500  0.0936
0.8000  0.0799
0.8500  0.0636
0.9000  0.0449
0.9500  0.0237
1.0000  0.0000
/\relax
}\relax
\Green{\relax 
\setdashes <5pt>
\plot
0.0000  0.0134
0.0500  0.0266
0.1000  0.0382
0.1500  0.0484
0.2000  0.0572
0.2500  0.0645
0.3000  0.0704
0.3500  0.0748
0.4000  0.0778
0.4500  0.0793
0.5000  0.0793
0.5500  0.0779
0.6000  0.0751
0.6500  0.0708
0.7000  0.0650
0.7500  0.0578
0.8000  0.0492
0.8500  0.0390
0.9000  0.0275
0.9500  0.0145
1.0000  0.0000
/\relax
}\relax
%
\Red{\relax 
\setdashes <2pt>
\plot
0.0000  -0.1684
0.0500  -0.1855
0.1000  -0.1999
0.1500  -0.2117
0.2000  -0.2207
0.2500  -0.2270
0.3000  -0.2307
0.3500  -0.2317
0.4000  -0.2300
0.4500  -0.2256
0.5000  -0.2185
0.5500  -0.2087
0.6000  -0.1963
0.6500  -0.1812
0.7000  -0.1633
0.7500  -0.1428
0.8000  -0.1196
0.8500  -0.0938
0.9000  -0.0652
0.9500  -0.0339
1.0000  0.0000
/\relax
}\relax
\endpicture
%
}
%
\vskip 15pt
\hbox to \hsize{\copy\figurefour\hss\copy\figurefive\hss\copy\figuresix}
\vskip 15pt
%%%%%%%%%%%%%%%%%%%%%%%  end of q_mixed plots  %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%  beginning of f_fiti plots  %%%%%%%%%%%%%%%%%%%%
% Now start the f(u) plots
\xfigdim = 0.87true in
\yfigdim = 2.25true in
%
\setbox\figureseven=\vbox{\hsize=\xfigdim   % This box is for f_fiti_alpha=0.5
% colours follow those of the matlab pictures
% This is for fixed point scheme and $f(u))$, $\alpha = 0.5$
\beginpicture
\scriptsize
  \setcoordinatesystem units <\xfigdim,\yfigdim>  point at 0 -1.5
  \setplotarea x from 0 to 2, y from -0.04 to 0.51
  \axis bottom shiftedto y=0 ticks short numbered from 0 to 2 by 0.5 /
  \axis left ticks short unlabeled from 0.0 to 0.5 by 0.1 /
  \put{{\sevenrm 0.5}} [l] at 0.04 0.5
  %\put{{\sevenrm All $\times 10^{-3}$}} left at 0.02 1.5
  %\put {{\sevenrm $q_{err}$, $\alpha=0.99$}} [rb] at 0.96 0.05
\setquadratic
\setlinear
\setdashes <3pt>
% colours follow those of the matlab pictures
\setdashes <3pt>
\setsolid
\Black{\relax  % exact values
\plot
0.0000  0.0000
0.1005 -0.0099
0.2010 -0.0193
0.3015 -0.0274
0.4020 -0.0337
0.5025 -0.0376
0.6030 -0.0384
0.7035 -0.0355
0.8041 -0.0284
0.9046 -0.0164
1.0051 0.0010
1.1056 0.0246
1.2061 0.0548
1.3066 0.0924
1.4071 0.1379
1.5076 0.1919
1.6081 0.2551
1.7086 0.3280
1.8092 0.4112
1.9097 0.5055
/\relax
}
%
\Blue{\relax  
\setdashes <8pt>
\plot
0.0000 0.0000
0.1005 -0.0099
0.2010 -0.0192
0.3015 -0.0273
0.4020 -0.0336
0.5025 -0.0374
0.6030 -0.0382
0.7035 -0.0353
0.8041 -0.0282
0.9046 -0.0162
1.0051 0.0012
1.1056 0.0248
1.2061 0.0550
1.3066 0.0926
1.4071 0.1381
1.5076 0.1921
1.6081 0.2552
1.7086 0.3281
1.8092 0.4113
1.9097 0.5055
/\relax
}\relax
%
\Green{\relax  
\setdashes <5pt>
\plot
0.0000 0.0000
0.1005 -0.0102
0.2010 -0.0198
0.3015 -0.0282
0.4020 -0.0347
0.5025 -0.0388
0.6030 -0.0399
0.7035 -0.0373
0.8041 -0.0304
0.9046 -0.0186
1.0051 -0.0013
1.1056 0.0221
1.2061 0.0522
1.3066 0.0897
1.4071 0.1351
1.5076 0.1891
1.6081 0.2522
1.7086 0.3252
1.8092 0.4085
1.9097 0.5029
/\relax
}\relax
%
\Red{\relax  
\setdashes <2pt>
\plot
0.0000 0.0000
0.1005 -0.0071
0.2010 -0.0145
0.3015 -0.0215
0.4020 -0.0274
0.5025 -0.0316
0.6030 -0.0332
0.7035 -0.0317
0.8041 -0.0262
0.9046 -0.0163
1.0051 -0.0010
1.1056 0.0201
1.2061 0.0480
1.3066 0.0831
1.4071 0.1263
1.5076 0.1783
1.6081 0.2396
1.7086 0.3110
1.8092 0.3933
/\relax
}\relax  % end of colour red
\endpicture
} % end of box
%
\setbox\figureeight=\vbox{\hsize=\xfiglen   % This box is for f_fiti_alpha=0.7
\beginpicture
\scriptsize
  \setcoordinatesystem units <\xfigdim,\yfigdim>  point at 0 -1.5
  \setplotarea x from 0 to 2, y from -0.1 to 0.5
  \axis bottom shiftedto y=0 ticks short numbered from 0 to 2 by 0.5 /
  \axis left ticks short unlabeled from 0 to 0.5 by 0.1 /
  \put {$0.5$} [l] at 0.04 0.5 
  %\put{{\sevenrm All $\times 10^{-3}$}} left at 0.02 1.5
  %\put {{\sevenrm $q_{err}$, $\alpha=0.99$}} [rb] at 0.96 0.05
\setquadratic
\setlinear
% colours follow those of the matlab pictures
% This is for fixed point scheme and $f(u)$, $\alpha = 0.7$
\setdashes <3pt>
\setsolid
\Black{\relax  % exact values
\plot
0.0000 0.0000
0.1005  -0.0099
0.2010  -0.0193
0.3015  -0.0274
0.4020  -0.0337
0.5025  -0.0376
0.6030  -0.0384
0.7035  -0.0355
0.8041  -0.0284
0.9046  -0.0164
1.0051  0.0010
1.1056  0.0246
1.2061  0.0548
1.3066  0.0924
1.4071  0.1379
1.5076  0.1919
1.6081  0.2551
1.7086  0.3280
1.8092  0.4112
1.9097  0.5055
/\relax
}
%
\Blue{\relax  
\setdashes <8pt>
\plot
0       0
0.1005  -0.0099
0.2010  -0.0192
0.3015  -0.0273
0.4020  -0.0336
0.5026  -0.0374
0.6031  -0.0382
0.7036  -0.0354
0.8041  -0.0283
0.9046  -0.0163
1.0051  0.0012
1.1056  0.0248
1.2061  0.0550
1.3066  0.0926
1.4072  0.1381
1.5077  0.1921
1.6082  0.2552
1.7087  0.3281
1.8092  0.4113
1.9097  0.5055
/\relax
}
%
%
\Green{\relax
\setdashes <5pt>
\plot
0       0
0.1005  -0.0116
0.2010  -0.0224
0.3015  -0.0318
0.4020  -0.0391
0.5026  -0.0438
0.6031  -0.0453
0.7036  -0.0430
0.8041  -0.0362
0.9046  -0.0245
1.0051  -0.0072
1.1056  0.0163
1.2061  0.0466
1.3066  0.0843
1.4072  0.1299
1.5077  0.1841
1.6082  0.2474
1.7087  0.3205
1.8092  0.4039
1.9097  0.4982
/\relax
}
%
\Red{\relax 
\setdashes <2pt>
\plot
0       0
0.1005  -0.0110
0.2010  -0.0219
0.3015  -0.0319
0.4020  -0.0405
0.5026  -0.0469
0.6031  -0.0505
0.7036  -0.0506
0.8041  -0.0466
0.9046  -0.0377
1.0051  -0.0233
1.1056  -0.0028
1.2061  0.0246
1.3066  0.0594
1.4072  0.1024
1.5077  0.1543
1.6082  0.2156
1.7087  0.2871
1.8092  0.3694
1.9097  0.4632
/\relax
}
\endpicture
} % end of box 8
%
\setbox\figurenine=\vbox{\hsize=\xfiglen   % This box is for f_fiti_alpha=0.99
\beginpicture
\scriptsize
  \setcoordinatesystem units <\xfigdim,\yfigdim>  point at 0 -1.5
  %\axis left ticks short numbered from 0 to 0.08 by 0.02 /
  \setplotarea x from 0 to 2, y from -0.1 to 0.5
  \axis bottom shiftedto y=0 ticks short numbered from 0 to 2 by 0.5 /
  \axis left ticks short unlabeled from 0 to 0.5 by 0.1 /
  \put {0.5} [l] at 0.04 0.5
  %\put{{\sevenrm All $\times 10^{-3}$}} left at 0.02 1.5
  %\put {{\sevenrm $q_{err}$, $\alpha=0.99$}} [rb] at 0.96 0.05
\setquadratic
\setlinear
% colours follow those of the matlab pictures
% This is for fixed point scheme and $f(u)$, $\alpha = 0.99$
%\setdashes <3pt>
\setsolid
\Black{\relax  % exact values
\plot
0.1005  -0.0100
0.2011  -0.0193
0.3016  -0.0274
0.4021  -0.0337
0.5027  -0.0376
0.6032  -0.0384
0.7038  -0.0355
0.8043  -0.0284
0.9048  -0.0164
1.0054  0.0011
1.1059  0.0247
1.2064  0.0550
1.3070  0.0926
1.4075  0.1381
1.5081  0.1922
1.6086  0.2554
1.7091  0.3283
1.8097  0.4117
1.9102  0.5060
/\relax
}
%
\Blue{\relax  
\setdashes <8pt>
\plot
0       0
0.1005  -0.0100
0.2011  -0.0193
0.3016  -0.0275
0.4021  -0.0338
0.5027  -0.0376
0.6032  -0.0385
0.7038  -0.0356
0.8043  -0.0285
0.9048  -0.0165
1.0054  0.0009
1.1059  0.0245
1.2064  0.0547
1.3070  0.0923
1.4075  0.1378
1.5081  0.1918
1.6086  0.2550
1.7091  0.3279
1.8097  0.4111
1.9102  0.5053
/\relax
}
%
\Green{\relax 
\setdashes <5pt>
\plot
0       0
0.1005  -0.0145
0.2011  -0.0277
0.3016  -0.0390
0.4021  -0.0478
0.5027  -0.0536
0.6032  -0.0559
0.7038  -0.0541
0.8043  -0.0476
0.9048  -0.0359
1.0054  -0.0185
1.1059  0.0052
1.2064  0.0358
1.3070  0.0738
1.4075  0.1197
1.5081  0.1742
1.6086  0.2376
1.7091  0.3107
1.8097  0.3939
1.9102  0.4879
/\relax
}
%
\Red{\relax  
\setdashes <2pt>
\plot
0       0
0.1005  -0.0172
0.2011  -0.0337
0.3016  -0.0487
0.4021  -0.0617
0.5027  -0.0719
0.6032  -0.0789
0.7038  -0.0819
0.8043  -0.0803
0.9048  -0.0735
1.0054  -0.0608
1.1059  -0.0417
1.2064  -0.0155
1.3070  0.0185
1.4075  0.0609
1.5081  0.1123
1.6086  0.1733
1.7091  0.2446
1.8097  0.3269
1.9102  0.4206
/\relax
}\relax
\endpicture
} % end of box 9
%
\scrollmode
\xfigdim = 0.87true in
\yfigdim = 0.15true in
\setbox\figureten=\vbox{\hsize=\xfiglen   % This box is for f_mix=0.5
 \beginpicture
 \scriptsize
   \setcoordinatesystem units <\xfigdim,\yfigdim>  point at 0 -1.5
   \setplotarea x from 0 to 2, y from -0.0 to 8
   \axis left ticks short unlabeled from 0 to 8 by 1 /
   \axis bottom shiftedto y=0 ticks short numbered from 0 to 2 by 0.5 /
  \put {8.0} left at 0.13 8
   %\put{{\sevenrm All $\times 10^{-3}$}} left at 0.02 1.5
   %\put {{\sevenrm $q_{err}$, $\alpha=0.99$}} [rb] at 0.96 0.05
%\setquadratic
 \setlinear
% colours follow those of the matlab pictures
% This is for fixed mixed scheme and $f(u)$, $\alpha = 0.5$
% \setdashes <3pt>
% \setsolid
\Black{\relax  % exact values
 \plot
 0       0
 0.1005  0.0010
 0.2010  0.0081
 0.3015  0.0274
 0.4020  0.0650
 0.5025  0.1269
 0.6030  0.2193
 0.7035  0.3482
 0.8040  0.5198
 0.9045  0.7401
 1.0050  1.0152
 1.1055  1.3512
 1.2060  1.7542
 1.3065  2.2303
 1.4070  2.7856
 1.5075  3.4262
 1.6081  4.1582
 1.7086  4.9875
 1.8091  5.9205
 1.9096  6.9631
 /\relax
}\relax
%
\Blue{\relax  % 
\setdashes <8pt>
 \plot
 0       0
 0.1005  0.0010
 0.2010  0.0081
 0.3015  0.0274
 0.4020  0.0650
 0.5025  0.1269
 0.6030  0.2193
 0.7035  0.3483
 0.8040  0.5200
 0.9045  0.7403
 1.0050  1.0155
 1.1055  1.3517
 1.2060  1.7548
 1.3065  2.2311
 1.4070  2.7865
 1.5075  3.4273
 1.6081  4.1594
 1.7086  4.9890
 1.8091  5.9222
 1.9096  6.9650
 /\relax
}\relax
%
\Green{\relax  
\setdashes <5pt>
 \plot
 0       0
 0.1005  -0.0020
 0.2010  0.0038
 0.3015  0.0236
 0.4020  0.0634
 0.5025  0.1295
 0.6030  0.2279
 0.7035  0.3647
 0.8040  0.5461
 0.9045  0.7781
 1.0050  1.0670
 1.1055  1.4188
 1.2060  1.8397
 1.3065  2.3357
 1.4070  2.9130
 1.5075  3.5777
 1.6081  4.3360
 1.7086  5.1939
 1.8091  6.1576
 1.9096  7.2332
/ \relax
 }\relax
%
\Red{\relax 
\setdashes <2pt>
  \plot
  0.0     0.0
 0.1005  -0.0023
 0.2010  0.0080
 0.3015  0.0370
 0.4020  0.0909
 0.5025  0.1756
 0.6030  0.2972
 0.7035  0.4618
 0.8040  0.6755
 0.9045  0.9442
 1.0050  1.2742
 1.1055  1.6714
 1.2060  2.1419
 1.3065  2.6918
 1.4070  3.3272
 1.5075  4.0540
 1.6081  4.8785
 1.7086  5.8065
 1.8091  6.8443
 1.9096  7.9979
 /\relax
}\relax
\endpicture
} % end of box 10
%
\setbox\figureeleven=\vbox{\hsize=\xfiglen   % This box is for f_mix=0.7
\beginpicture
\scriptsize
  \setcoordinatesystem units <\xfigdim,\yfigdim>  point at 0 -1.5
  \axis left ticks short unlabeled from 0 to 8 by 1 /
  \setplotarea x from 0 to 2, y from -0.1 to 8
  \axis bottom shiftedto y=0 ticks short numbered from 0 to 2 by 0.5 /
  \axis left ticks short unlabeled from 0 to 8 by 1 /
  \put {8.0} left at 0.13 8
  %\put{{\sevenrm All $\times 10^{-3}$}} left at 0.02 1.5
  %\put {{\sevenrm $q_{err}$, $\alpha=0.7$}} [rb] at 0.96 0.05
\setquadratic
\setlinear
% colours follow those of the matlab pictures
% This is for fixed mixed scheme and $f(u)$, $\alpha = 0.7$
\setdashes <3pt>
\setsolid
\Black{\relax  % exact values
\plot
0       0
0.1005  0.0010
0.2010  0.0081
0.3015  0.0274
0.4020  0.0650
0.5025  0.1269
0.6030  0.2193
0.7035  0.3482
0.8040  0.5198
0.9045  0.7401
1.0050  1.0152
1.1055  1.3512
1.2060  1.7542
1.3065  2.2303
1.4070  2.7856
1.5075  3.4262
1.6081  4.1582
1.7086  4.9875
1.8091  5.9205
1.9096  6.9631
/\relax
}\relax
%
\Blue{\relax  
\setdashes <8pt>
\plot
0       0
0.1005  0.0010
0.2010  0.0081
0.3015  0.0274
0.4020  0.0650
0.5025  0.1269
0.6030  0.2193
0.7035  0.3483
0.8040  0.5200
0.9045  0.7403
1.0050  1.0155
1.1055  1.3517
1.2060  1.7548
1.3065  2.2311
1.4070  2.7865
1.5075  3.4273
1.6081  4.1594
1.7086  4.9890
1.8091  5.9222
1.9096  6.9650
/\relax
}\relax
%
%
\Green{\relax
\setdashes <5pt>
\plot
0       0
0.1005  -0.0020
0.2010  0.0038
0.3015  0.0236
0.4020  0.0634
0.5025  0.1295
0.6030  0.2279
0.7035  0.3647
0.8040  0.5461
0.9045  0.7781
1.0050  1.0670
1.1055  1.4188
1.2060  1.8397
1.3065  2.3357
1.4070  2.9130
1.5075  3.5777
1.6081  4.3360
1.7086  5.1939
1.8091  6.1576
1.9096  7.2332
/\relax
}\relax
\Red{\relax 
\setdashes <2pt>
\plot
0       0
0.1005  -0.0023
0.2010  0.0080
0.3015  0.0370
0.4020  0.0909
0.5025  0.1756
0.6030  0.2972
0.7035  0.4618
0.8040  0.6755
0.9045  0.9442
1.0050  1.2742
1.1055  1.6714
1.2060  2.1419
1.3065  2.6918
1.4070  3.3272
1.5075  4.0540
1.6081  4.8785
1.7086  5.8065
1.8091  6.8443
1.9096  7.9979
/\relax
}\relax
\endpicture
} % end of box 11
%
\setbox\figuretwelve=\vbox{\hsize=\xfiglen   % This box is for f_mix=0.99
\beginpicture
\scriptsize
  \setcoordinatesystem units <\xfigdim,\yfigdim>  point at 0 -1.5
  \setplotarea x from 0 to 2, y from 0 to 8
  \axis bottom shiftedto y=0 ticks short numbered from 0 to 2 by 0.5 /
  \axis left ticks short unlabeled from 0 to 8 by 1 /
  \put {8.0} left at 0.13 8
\setquadratic
\setlinear
% colours follow those of the matlab pictures
% This is for fixed mixed scheme and $f(u)$, $\alpha = 0.99$
\Black{\relax  % exact values
\plot
0.0       0.0
0.1005  0.0010
0.2010  0.0081
0.3015  0.0274
0.4020  0.0650
0.5025  0.1269
0.6030  0.2193
0.7035  0.3482
0.8040  0.5198
0.9045  0.7401
1.0050  1.0152
1.1055  1.3512
1.2060  1.7542
1.3065  2.2303
1.4070  2.7856
1.5075  3.4262
1.6081  4.1582
1.7086  4.9875
1.8091  5.9205
1.9096  6.9631
/\relax
}\relax
%
\Blue{\relax  % last iterate
\setdashes <8pt>
\plot
0       0
0.1005  0.0010
0.2010  0.0081
0.3015  0.0274
0.4021  0.0650
0.5026  0.1269
0.6031  0.2193
0.7036  0.3483
0.8041  0.5200
0.9046  0.7403
1.0051  1.0155
1.1057  1.3517
1.2062  1.7548
1.3067  2.2311
1.4072  2.7865
1.5077  3.4273
1.6082  4.1594
1.7087  4.9890
1.8092  5.9222
1.9098  6.9650
/\relax
}\relax
%
\Green{\relax  % exact values
\setdashes <5pt>
\plot
0       0
0.1005  -0.0020
0.2010  0.0038
0.3015  0.0236
0.4021  0.0634
0.5026  0.1295
0.6031  0.2279
0.7036  0.3647
0.8041  0.5461
0.9046  0.7781
1.0051  1.0670
1.1057  1.4188
1.2062  1.8397
1.3067  2.3357
1.4072  2.9130
1.5077  3.5777
1.6082  4.3360
1.7087  5.1939
1.8092  6.1576
1.9098  7.2332
/\relax
}\relax
%
\Red{\relax  
\setdashes <2pt>
\plot
0       0
0.1005  -0.0023
0.2010  0.0080
0.3015  0.0370
0.4021  0.0909
0.5026  0.1756
0.6031  0.2972
0.7036  0.4618
0.8041  0.6755
0.9046  0.9442
1.0051  1.2742
1.1057  1.6714
1.2062  2.1419
1.3067  2.6918
1.4072  3.3272
1.5077  4.0540
1.6082  4.8785
1.7087  5.8065
1.8092  6.8443
1.9098  7.9979
/\relax
}\relax
%
\endpicture
} % end of box 12

\hbox to \hsize{\copy\figureseven\hss\copy\figureeight\hss\copy\figurenine}
\vskip25 pt
\hbox to \hsize{\copy\figureten\hss\copy\figureeleven\hss\copy\figuretwelve}
%\hbox to \hsize{\copy\figureeleven\hss\copy\figuretwelve}





==> fonts.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% This is the file fonts.tex
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\font\tenrm=cmr10
\font\teni=cmmi10 \skewchar\teni='177
\font\tensy=cmsy10 \skewchar\tensy='60
\font\tenex=cmex10
\font\tenit=cmti10
\font\tensl=cmsl10
\font\tenbf=cmbx10
\font\tentt=cmtt10
%
\font\ninerm=cmr9
\font\ninei=cmmi9 \skewchar\ninei='177
\font\ninesy=cmsy9 \skewchar\ninesy='60
\font\nineit=cmti9
\font\ninesl=cmsl9
\font\ninebf=cmbx9
\font\ninett=cmtt9
%
\font\eightrm=cmr8
\font\eighti=cmmi8 \skewchar\eighti='177
\font\eightsy=cmsy8 \skewchar\eightsy='60
\font\eightit=cmti8
\font\eightsl=cmsl8
\font\eightbf=cmbx8
\font\eighttt=cmtt8
%
\font\sevenrm=cmr7
\font\seveni=cmmi7 \skewchar\seveni='177
\font\sevensy=cmsy7 \skewchar\sevensy='60
\font\sevenbf=cmbx7
\font\sevenit=cmmi7
\font\sevensl=cmmi7
\font\seventt=cmr7
%
\font\sixrm=cmr6
\font\sixi=cmmi6 \skewchar\sixi='177
\font\sixsy=cmsy6 \skewchar\sixsy='60
\font\sixbf=cmbx6
%
\font\fiverm=cmr5
\font\fivei=cmmi5 \skewchar\fivei='177
\font\fivesy=cmsy5 \skewchar\fivesy='60
\font\fivebf=cmbx5
%

%
\def\tenpoint{\def\rm{\fam0\tenrm}%
        \textfont0=\tenrm \scriptfont0=\sevenrm \scriptscriptfont0=\fiverm
        \textfont1=\teni \scriptfont1=\seveni \scriptscriptfont1=\fivei
        \textfont2=\tensy \scriptfont2=\sevensy \scriptscriptfont2=\fivesy
        \textfont3=\tenex \scriptfont3=\tenex \scriptscriptfont3=\tenex
        \def\it{\fam\itfam\tenit}%
        \textfont\itfam=\tenit
        \def\sl{\fam\slfam\tensl}%
        \textfont\slfam=\tensl
        \def\bf{\fam\bffam\tenbf}%
        \textfont\bffam=\tenbf \scriptfont\bffam=\sevenbf
                \scriptscriptfont\bffam=\fivebf
        \def\tt{\fam\ttfam\tentt}%
        \textfont\ttfam=\tentt
        \normalbaselineskip=12pt%
        \let\sc=\eightrm        % Small caps
        \setbox\strutbox=\hbox{\vrule height8.5pt depth3.5pt width0pt}%
        \normalbaselines\rm}
%
\def\ninepoint{\def\rm{\fam0\ninerm}%
        \textfont0=\ninerm \scriptfont0=\sixrm \scriptscriptfont0=\fiverm
        \textfont1=\ninei \scriptfont1=\sixi \scriptscriptfont1=\fivei
        \textfont2=\ninesy \scriptfont2=\sixsy \scriptscriptfont2=\fivesy
        \textfont3=\tenex \scriptfont3=\tenex \scriptscriptfont3=\tenex
        \def\it{\fam\itfam\nineit}%
        \textfont\itfam=\nineit
        \def\sl{\fam\slfam\ninesl}%
        \textfont\slfam=\ninesl
        \def\bf{\fam\bffam\ninebf}%
        \textfont\bffam=\ninebf \scriptfont\bffam=\sixbf
                \scriptscriptfont\bffam=\fivebf
        \def\tt{\fam\ttfam\ninett}%
        \textfont\ttfam=\ninett
        \normalbaselineskip=11pt%
        \let\sc=\sevenrm        % Small caps
        \setbox\strutbox=\hbox{\vrule height8pt depth3pt width0pt}%
        \normalbaselines\rm}
%
\def\eightpoint{\def\rm{\fam0\eightrm}%
        \textfont0=\eightrm \scriptfont0=\sixrm \scriptscriptfont0=\fiverm
        \textfont1=\eighti \scriptfont1=\sixi \scriptscriptfont1=\fivei
        \textfont2=\eightsy \scriptfont2=\sixsy \scriptscriptfont2=\fivesy
        \textfont3=\tenex \scriptfont3=\tenex \scriptscriptfont3=\tenex
        \def\it{\fam\itfam\eightit}%
        \textfont\itfam=\eightit
        \def\sl{\fam\slfam\eightsl}%
        \textfont\slfam=\eightsl
        \def\bf{\fam\bffam\eightbf}%
        \textfont\bffam=\eightbf \scriptfont\bffam=\sixbf
                \scriptscriptfont\bffam=\fivebf
        \def\tt{\fam\ttfam\eighttt}%
        \textfont\ttfam=\eighttt
        \normalbaselineskip=9pt%
        \let\sc=\sixrm  % Small caps
        \setbox\strutbox=\hbox{\vrule height7pt depth2pt width0pt}%
        \normalbaselines\rm}
%
\def\sevenpoint{\def\rm{\fam0\sevenrm}%
        \textfont0=\sevenrm \scriptfont0=\fiverm \scriptscriptfont0=\fiverm
        \textfont1=\seveni \scriptfont1=\fivei \scriptscriptfont1=\fivei
        \textfont2=\sevensy \scriptfont2=\fivesy \scriptscriptfont2=\fivesy
        \textfont3=\tenex \scriptfont3=\tenex \scriptscriptfont3=\tenex
        \def\it{\fam\itfam\sevenit}%
        \textfont\itfam=\sevenit
        \def\sl{\fam\slfam\sevensl}%
        \textfont\slfam=\sevensl
        \def\bf{\fam\bffam\sevenbf}%
        \textfont\bffam=\sevenbf \scriptfont\bffam=\fivebf
                \scriptscriptfont\bffam=\fivebf
        \def\tt{\fam\ttfam\seventt}%
        \textfont\ttfam=\seventt
        \normalbaselineskip=8pt%
        \let\sc=\fiverm  % Small caps
        \setbox\strutbox=\hbox{\vrule height6pt depth2pt width0pt}%
        \normalbaselines\rm}

